Enumerating Error Bounded Polytime Algorithms Through Arithmetical Theories

We consider a minimal extension of the language of arithmetic, such that the bounded formulas provably total in a suitably-defined theory \`a la Buss (expressed in this new language) precisely capture polytime random functions. Then, we provide two new characterizations of the semantic class BPP obtained by internalizing the error-bound check within a logical system: the first relies on measure-sensitive quantifiers, while the second is based on standard first-order quantification. This leads us to introduce a family of effectively enumerable subclasses of BPP, called BPP_T and consisting of languages captured by those probabilistic Turing machines whose underlying error can be proved bounded in the theory T. As a paradigmatic example of this approach, we establish that polynomial identity testing is in BPP_T where T=$\mathrm{I}\Delta_0+\mathrm{Exp}$ is a well-studied theory based on bounded induction.

==> relatedwork.tex <==


%While the characterization of complexity classes through logic – and especially via bounded arithmetic \cite{Buss98} –
%is a vast research domain, the literature does not offer many such contributions about  probabilistic complexity classes.
%
While several recursion-theoretic characterizations of the syntactic class $\mathbf{PP}$ can be found  in~\cite{DalLagoKahleOitavem21,DalLagoKahleOitavem22},
existing characterizations of $\mathbf{BPP}$ rely on some  external, semantic condition  \cite{DalLagoParisenToldin,Scedrov}.
%
In particular,  
Eickmeyer and Grohe \cite{Grohe} provide a semantic characterization of $\BPP$ in a logic with fixed-point operators and a special counting quantifier, %coupled 
associated with a probabilistic semantics not too different from the quantitative interpretation we present in Section~\ref{sec:FAtoRC}. 
Beyond the previously discussed \cite{Jerabek}, Je\v{r}\'abek provides in \cite{JerabekAPAL} characterizations in bounded arithmetics of other (both syntactic and semantic) randomized classes, such as $\mathbf{ZPP}, \mathbf{RP}$ and $\mathbf{coRP}$.
Finally, \cite{Scedrov} defines a higher-order language for polytime oracle recursive functions based on an adaptation of Bellantoni-Cook's safe recursion.
%
%By contrast, \cite{Jerabek} studies a syntactic approach to probabilistic polytime programs in the context of bounded arithmetics and introduces a notion of ``definable $\BPP$-problem'', relative to some bounded theory and based on an arithmetical encoding of
%approximate counting problems.
%%
%Then, an intriguing question is whether such syntactically definable $\BPP$-problems can be related to the syntactic classes $\BPP_{T}$ we define in Section~\ref{sec:SSBPP}.

%

%
%\cite{Grohe} characterization of BPP in a logic with fixed-point operators and a special counting quantifier (Rescher quantifier) extended with a probabilistic semantics not too different from our quantitative semantics.
%
%\cite{Jerabek} encoding approximate counting in bounded arithmetic to formalize properties of BPP programs (although not a characterization of BPP in Buss' sense).
%
%\cite{Scedrov} a higher-order language for polytime oracle recursive functions based on an adaptation of Bellantoni-Cook's safe recursion.

